State Selection Algorithms and Their Impact on The Performance of Stateful Network Protocol Fuzzing

The statefulness property of network protocol implementations poses a unique challenge for testing and verification techniques, including Fuzzing. Stateful fuzzers tackle this challenge by leveraging state models to partition the state space and assist the test generation process. Since not all states are equally important and fuzzing campaigns have time limits, fuzzers need effective state selection algorithms to prioritize progressive states over others. Several state selection algorithms have been proposed but they were implemented and evaluated separately on different platforms, making it hard to achieve conclusive findings. In this work, we evaluate an extensive set of state selection algorithms on the same fuzzing platform that is AFLNet, a state-of-the-art fuzzer for network servers. The algorithm set includes existing ones supported by AFLNet and our novel and principled algorithm called AFLNetLegion. The experimental results on the ProFuzzBench benchmark show that (i) the existing state selection algorithms of AFLNet achieve very similar code coverage, (ii) AFLNetLegion clearly outperforms these algorithms in selected case studies, but (iii) the overall improvement appears insignificant. These are unexpected yet interesting findings. We identify problems and share insights that could open opportunities for future research on this topic.

==> Sections/AFLNetMCTS.tex <==
\section{\AFLNetLegion MCTS} \label{sec: aflnetlegion mcts}

\AFLNetLegion proposes a principled way to fuzz stateful servers.
Specifically, it models the state of servers within a variation of the MCTS framework proposed by a previous work \cite{Legion}.
This section describes the key modelling decisions, 
respectively the tree nodes (\cref{subsec: tree nodes}) and the tree construction (\cref{subsec: tree construction}),
to adopt the framework.



\subsection{Tree Nodes} \label{subsec: tree nodes}
Tree nodes are designed to allow \AFLNetLegion to fuzz the server from past snapshots
preferred by the MCTS framework.

Each snapshot of the server under test (SUT) is identified by a sequence of response codes
received during fuzzing.
The root of the tree represents the initial state of the server (denoted by a dummy code `0'), 
and every child node corresponds to a response code received after its parent code.
Each snapshot can be reproduced by the 
{\color{red} interesting (may delete, depending on the experiment results)} 
request sequence saved in the node.

To facilitate MCTS selection,
each node also records the statistics of the corresponding server state,
including the selection count and reward of the node, and of each request sequence.

\AFLNetLegion's nodes come in three types for different purposes.
For example, some response code sequences are triggered by a single request, 
in which case we can only reproduce the state represented by the last code in the sequence.
The last code of such sequence is represented by a \WhiteNode 
while the others are represented by \BlackNodes. 
A \GoldenNode is attached to each \WhiteNode, 
representing the option of launching fuzzing from the \WhiteNode.


\subsection{Tree Construction} \label{subsec: tree construction}
\begin{figure*}[ht!]
    \centering
    \input{MCTS-Phases.tex}
    \vspace*{-.3cm}
    \caption{The four stages of (each iteration of) \Legion's MCTS algorithm.}
    \label{fig: legion phases}
  \end{figure*}

  \cref{fig: legion phases} illustrates how \AFLNetLegion
explores the tree-structured search space in its variation of MCTS:
Each iteration of the search algorithm proceeds in four stages.
In \cref{fig: legion phases}, bold lines highlight the actions in each stage.
Solid thin lines and nodes represent paths and code blocks that have been
covered and integrated into the tree.
The four stages are as follows:

\bparagraph{Selection.}
The selection stage consists of two steps in a row: Tree node selection and Seed selection.
The tree node selection descends from the root node 
by recursively applying the \textit{selection policy}, until it reaches a \GoldenNode.
Then it applies the selection policy on all the request sequences stored in the tree node to find one to fuzz.

\bparagraph{Simulation.}

Like \AFLNet, \AFLNetLegion adopts \AFL for fuzzing.

\AFLNet splits each request sequence into three parts,
the prefix $M1$ consists the requests that can reproduce the state of the server 
corresponding to the state selected,
$M2$ contains all requests after $M1$ before the server transits to a new state,
and $M3$ stores all subsequent requests in the sequence.

Inherited from the \Legion's MCTS algorithm,
\AFLNetLegion preserves $M1$ and mutates both $M2$ and $M3$ to generate new request sequences.

\bparagraph{Expansion.}
Inherited from the MCTS framework of \Legion, 
\AFLNetLegion maps each observed response code sequence to a path of corresponding tree nodes.
As mentioned, only the last code of each subsequence of codes triggered by a single request 
will be created as a \WhiteNode 
while all its ancestors of the same subsequence (if any) will be added as \BlackNodes.
Again, a \GoldenNode will be attached to each \WhiteNode.

\bparagraph{Backpropagation.}
This step updates the statistics recorded in the tree to assist future decision making.

Specifically, 
It adds one to the selection count of each node chosen in the Selection step to record the decision,
and adds the number of new response code sequences observed in the Simulation step 
to the reward in each node of such sequence.

Similarly, for each new path selected or found by fuzzing the selected request sequence, 
this step respectively increases the selection count or reward count of that request sequence by one.





point the readers to related work for a detailed comparison between aflnet aflnetlegion and legion

==> Sections/Algorithm.tex <==
\section{Algorithm} \label{sec: aflnetlegion - algorithm}
% To demonstrate the impact of selection algorithms, 
% we implemented a principled algorithm \AFLNetLegion on the engineering basis of \AFLNet.
% \AFLNetLegion adopts the MCTS algorithm proposed by \Legion, which proven useful on ordinary testing.
Based on the observation from \cref{sec: aflnetlegion - overview},
\AFLNetLegion proposes a principled way to fuzz stateful servers.
Specifically, it models the state of servers within 
a variation of the MCTS framework proposed by \Legion.
This framework differs from \AFLNet in two ways.
In addition to the fine-grain model demonstrated in \cref{sec: aflnetlegion - overview},
it also adopts a principled UCT function to evaluate each state,
rather than relying on an empirical function as \AFLNet.
This section describes the key modelling decisions, respectively 
the tree nodes (\cref{subsec: tree nodes}),
the tree construction (\cref{subsec: tree construction}),
and the selection policy of nodes (\cref{subsec: selection policy}),
to adopt the framework.


\subsection{Tree Nodes} \label{subsec: tree nodes}
Tree nodes are designed to allow \AFLNetLegion to fuzz the server from past snapshots
preferred by the MCTS framework.

Each snapshot of the server under test (SUT) is identified by a sequence of response codes
received during fuzzing.
The root of the tree represents the initial state of the server (denoted by a dummy code `0'), 
and every child node corresponds to a response code received after its parent code.
Each snapshot can be reproduced by the \textit{interesting} request sequence saved in the node.
A request is considered interesting to a node if it finds a new child of the node.
This is because,
under the MCTS paradigm,
we consider all requests that produce the same response code from the same server state
as an identical action,
and only save (the first) one of them to avoid duplication.

To facilitate MCTS selection,
each node also records the statistics of the corresponding server state,
including the selection count and reward of the node, and of each request sequence.

\AFLNetLegion's nodes come in three types for different purposes.
For example, in some cases,
one request can trigger multiple response codes in a row,
in which case we can only reproduce the server state represented by the last code in them.
The last code of them is represented by a \white node 
while the others are represented by \black nodes.
A \golden node is attached to each \white node,
representing the option of launching fuzzing from the latter.

Note that the \red node from \Legion is not applicable in \AFLNetLegion,
since symbolic execution is not available for external servers.
Consequently,
we can never know if all children of a node have been found,
which highlights the necessity of a principled selection algorithm
(\cref{subsec: selection policy})
that can upper-bound the expected loss due to not selecting the best request sequence to fuzz.

\subsection{Tree Construction} \label{subsec: tree construction}
\begin{figure*}[ht!]
    \centering
    \input{MCTS-Phases.tex}
    \vspace*{-.3cm}
    \caption{The four stages of (each iteration of) \AFLNetLegion's MCTS algorithm, Based on the figure of four stages of \Legion}
    \label{fig: aflnetlegion phases}
  \end{figure*}

  \cref{fig: aflnetlegion phases} illustrates how \AFLNetLegion
explores the tree-structured search space in its variation of MCTS:
Each iteration of the search algorithm proceeds in four stages.
In \cref{fig: aflnetlegion phases}, bold lines highlight the actions in each stage.
Solid thin lines and nodes represent paths and code blocks that have been
covered and integrated into the tree.
The four stages are as follows:

\bparagraph{Selection.}
The selection stage consist of two steps in a row: 
Tree node selection and seed request sequence selection.
The tree node selection descends from the root node 
by recursively applying the \textit{selection policy}, until it reaches a \golden node.
Then it applies the selection policy on 
all the request sequences stored in the tree node to find an seed to mutate.

\bparagraph{Simulation.}
% Like \AFLNet, \AFLNetLegion adopts \AFL for fuzzing.
The simulation stage explores different behaviour of the server after the selected state.
Among the three seed request sequence sections marked by \AFLNet
(discussed in \cref{sec: aflnetlegion - background}),
\AFLNetLegion replays the prefix section
and mutates both the candidate and the suffix sections.
This design decision follows the random policy of the MCTS paradigm.

\bparagraph{Expansion.}
The expansion stage records all newly discovered response sequence into the tree.
Inherited from the MCTS framework of \Legion,
\AFLNetLegion maps each observed response code sequence to a path of corresponding tree nodes.
When a new response code subsequence is found,
it adds each of the new code as a new child node of the previous one,
and saves the corresponding request sequence to the parent of the first new node
and every new descendants.
It also marks the three sections of the new request sequence when saving it to each node
so that the sequence can be reused in the future simulation stages.
As mentioned,
when a single request triggers multiple response codes in a row,
only the last code of such subsequence will be created as a \white node
while all its ancestors of the same subsequence (if any) will be added as \black nodes.
Again, a \golden node will be attached to each \white node.

\bparagraph{Backpropagation.}
This stage updates the statistics recorded in the tree to assist future decision making.
For each mutant executed in the simulation stage,
\AFLNetLegion increases the \textit{past selection count} of 
each node chosen in the selection stage by one to
discourage selecting the same nodes too often.
For each new response code sequence observed,
it increases the \textit{past discovery count}
of every new node and the parent of the first new node,
to encourage selecting them in the future.
The usage of these two counts are discussed in \cref{subsec: selection policy}.

% Similarly,
% for each new path selected or found by fuzzing the selected input,
% this step respectively increases the selection count or reward count of that input by one.

% point the readers to related work for a detailed comparison between aflnet aflnetlegion and legion

\subsection{Selection policy} \label{subsec: selection policy}
\AFLNetLegion's selection policy takes charge of 
choosing tree nodes and seed request sequences based on their statistics
in the selection stage of MCTS.

It estimates the productivity of a program state regarding finding more uncover server states
with the same two statistics as \AFLNet,
namely,
\textit{past discovery count} and \textit{past selection count}.
The former represents the number of response code sequences found
under the target program state,
higher discovery indicates high productivity of the state.
The latter stands for the number of times the target state has been selected for fuzzing,
less selection implies high uncertainty about the state.
Together, they attempt to
balance exploitation of the states that appear to be most productivity based on past experience, 
against exploration of less-well understood parts of the program
where productivity (path/response code sequence discovery) are less certain.


\begin{equation}
% \begin{gather*}
  \UCT(N) =  
  \begin{cases}
    \infty  & S=0\\
    \frac{D}{S} + \rho\sqrt{ \frac{2\ln{P_S}}{S} } & S > 0
  \end{cases}
% \end{gather*}
\label{eqn: UCT}
\end{equation}

{\color{red} move the above to background?}

% The reason behind this heuristic is explained in detail in \Legion.
Different from \AFLNet (who relies on empirical formulas),
\AFLNetLegion borrows \cref{eqn: UCT}  from \Legion
to evaluate both tree nodes and request sequences:
For node evaluation,
$D$, $S$, and $P_S$ respectively denotes 
\textit{past discovery count} of the node,
\textit{past selection count} of the node,
and \textit{past selection count} of the node $N$'s parent node $P$.
For seed evaluation,
$D$, $S$, and $P_S$ respectively denotes 
\textit{past discovery count} of the seed,
\textit{past selection count} of the seed,
and \textit{past selection count} of the seed's belonging simulation node $P$.
The discovery count of a seed records 
the number of new request sequences found by mutating the seed,
its selection count records the number of times the seed has been selected for mutation.


==> Sections/Overview.tex <==
\section{Overview} \label{sec: aflnetlegion - overview}

To analyse the impact of server modelling
and request sequence algorithm
on coverage performance,
this section
uses \AFLNet as the baseline
to compare with a principled guideline algorithm on external protocol fuzzing.
We name this guideline algorithm \AFLNetLegion
as it builds upon the implementation of \AFLNet and
follows \Legion's variation of the Monte Carlo tree search algorithm
to formulate the problem of selecting request sequence as a sequential decision making process.


\subsection{AFLNet's state machine model}

\AFLNet's model and algorithm (explained in \cref{sec: aflnetlegion - background - aflnet})
suffers from two weaknesses.
% to fuzz external servers with sequences of requests.
First, its state machine model groups the request sequence only by individual response codes 
without distinguishing their prefixes.
Such coarse-grained partition complicates request sequence selection within each state
and leads to unreliable estimation of the potential of each state.
Second, its request sequence selection algorithm lacks
a systematic and principled guidance
in the large and complex input space under the uncertainty of the external server implementation.

\begin{figure*}[ht]
    
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \lstinputlisting[style=aflnet]{RequestSeqs1.tex}
    \caption{Request sequence 1: \glob before creating directory and file}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
    \lstinputlisting[style=aflnet, emph={NLST}]{RequestSeqs2.tex}
    \caption{Request sequence 2: \glob after creating directory and file}
    \end{subfigure}
    \caption{Two sample request sequences involving globbing with \texttt{NLST}}
    \label{fig: RequestSeqs}
\end{figure*}

\cref{fig: RequestSeqs} exemplifies a case study that illustrates
how a coarse-grained input space partition from the state machine model
diminishes the effect of request sequence selection algorithms.
% how a principle approach from \Legion mitigates these two weaknesses.
Both sequences contains the same requests, but in different orders:
In sequence 1 on the left, the \NLST request is executed 
before creating any file or directory,
while in sequence 2 on the right, a directory and a file are created before 
executing the same \NLST command.
As a result,
the \NLST command in sequence 2 is more interesting than sequence 1 to fuzz
regarding covering much more code of the \glob library
when the server attempts to expand the asterisk (\texttt{*}).
A rigorous model of the server should distinguish the difference between the two sequences
so that the selection algorithm can later learn sequence 2 is more interesting than 1.

This is a typical example where
a more rigorous model
plays a more important role in improving the coverage performance of \AFLNet
than a cleverer request sequence selection algorithm.
\cref{fig: AFLNet state machine} illustrates the state machine of the server's responses to
two sequences of requests.
The initial server state is represented by a dummy code 0,
and each following state is identified with the response code of the latest command.
% The blue and red line respectively represent the response sequence from sequence 1 and 2.
Note that the \texttt{FTP} server responses the same code (\texttt{250}) to successful 
\NLST and \texttt{STOR} commands, 
hence the state machine is unable to distinguish their states.

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/AFLNetModel}
%     % \input{Figures/AFLNetModel.tex}
%     \vspace*{-.3cm}
%     \caption{\AFLNet's state machine model of \cref{fig: RequestSeqs}}
%     \label{fig: AFLNet state machine}
% \end{figure*}

% \begin{figure*}[ht!]
%     \centering
%     % \includegraphics[width=\linewidth]{Figures/AFLNetModel}
%     \input{Figures/AFLNetModel.tex}
%     \vspace*{-.3cm}
%     \caption{\AFLNet's state machine model of \cref{fig: RequestSeqs}}
%     \label{fig: AFLNet state machine}
% \end{figure*}

\AFLNet's state machine models limits the performance of selection algorithms,
because it partitions the input space at a coarse-gain level.
For example, this model groups both request sequences in state \texttt{250}.
As a result,
the boring noise request sequence 1 lowers the estimated value of the state
and consequently reduces the chance of selecting the interesting sequence 2.
Similarly, with more request sequences generated later,
it may group more noise request sequences and further complicates request sequence selection in the state,
such as
\texttt{USER -> PASS -> NLST -> NLST} and 
\texttt{USER -> PASS -> NLST -> NLST -> MKD -> STOR -> NLST}.
In addition, in the latter sequence,
the selection algorithm will also have difficulty deciding which \NLST to mutate.


\subsection{A principled tree model} \label{sec: aflnetlegion - overview - a principled tree model}
Observing the weakness of \AFLNet's graph model,
\AFLNetLegion proposes the following two improvements:
a) a more fine-grained request sequence partition with a tree model;
b) a more systematic request sequence selection algorithm for external server fuzzing varited from \Legion.

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{Figures/AFLNetModel.tex}
        \vspace*{-.3cm}
        \caption{\AFLNet's state machine model}
        \label{fig: AFLNet state machine}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{Figures/AFLNetLegionModel.tex}
        \vspace*{-.3cm}
        \caption{\AFLNetLegion's tree model}
        \label{fig: AFLNetLegion tree}
    \end{subfigure}
    \caption{Two models of the request sequences in \cref{fig: RequestSeqs}\\
            the bold font \textbf{\texttt{NLST}} is the interesting one from \AFLNetLegion}
\end{figure*}

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/AFLNetLegionModel}
%     % \input{Figures/AFLNetModel.tex}
%     \vspace*{-.3cm}
%     \caption{\AFLNet's state machine model of \cref{fig: RequestSeqs}}
%     \label{fig: AFLNet state machine}
% \end{figure*}

\cref{fig: AFLNetLegion tree} illustrates \AFLNetLegion's tree model.
The tree root is a again dummy node representing the initial state of the server,
while every child node corresponds to subsequent response code of the latest command.
Every node is identified with a unique partial response code sequence.
Each stores the statistics and request sequences of 
the response code sequence observed so far that pass through that node.

The tree model allows a more fine-grained input space partition,
because it distinguishes two nodes not only by their own response code,
but also with their prefixes.
For example,
node \texttt{250''} is clearly distinguished from other nodes with the same response code 
(e.g. \texttt{250}, \texttt{250'}, \texttt{250'''}).
This ensures the mode will 
only group request sequence 2 or similar interesting sequences with the same prefix into the node.
Consequently,
no noise request sequence will 
undermine the actual statistics of each node or complicate its request sequence selection.
\cref{sec: aflnetlegion - algorithm} explains 
the technical detail of the construction and usage of the tree model.
% \subsection{A principled algorithm} \label{sec: aflnetlegion - overview - a principled algorithm}


{\color{red}
\AFLNetLegion's selection algorithm is similar to \AFLNet's.
Both of them attempt to balance exploration and exploitation.
The only difference is in their score function:
\AFLNetLegion uses the more principled UCT function,
while \AFLNet uses an emperical formula.
Not sure if it is meaningful/necessary to discuss them here.
}

==> Sections/PracticalConsiderations.tex <==
\section{Practical Considerations} \label{sec: practical considerations}
{\color{red}
Not important, maybe mention them in the experiment section?
Can cut them to save space.
}

\subsection{Hyper-parameters}

\bparagraph{Rho.} 
We selected $\rho=0.0025$ based on \Legion.

\bparagraph{Tree depth.} 
We only consider the first $200$ response code in each sequence.

% \bparagraph{Execution timeout.}
% Each server execution times out after {\color{red}$X$ minutes}.

\bparagraph{Fuzz M3.} \label{par: fuzz m3}
As mentioned in \cref{subsec: tree construction}, 
while \AFLNet only mutates $M2$,
\AFLNetLegion mutates both $M2$ and $M3$ according to the MCTS algorithm proposed by \Legion.

==> Sections/RelatedWork.tex <==
\section{Related Work}
\label{sec: aflnetlegion - related work}

Many researchers proposed different server modelling and query selection algorithms
under different implementations.
This chapter disentangles three aspects of external server fuzzing,
namely implementation, server modelling, and query selection algorithm.
In this chapter,
we control the first aspect
to examine the role and impact of the latter two aspects in active learning,
i.e. learning the server model and refining selection algorithm while actively querying the SUT.
At the high-level, 
we consider server modelling as a process of input space partition
to further assist the query sequence selection algorithm for SUT exploration.
% Because otherwise the selection space would be too large and 
% there will be too many input sequence to try out.

Existing techniques tend to model the the SUT with state machines.
A state machine is a graph consisting of a finite number of states and transitions between states.
Here client queries of predefined syntax/format correspond to the transitions
and different server statuses triggered by the queries are abstracted to states.
Many works use a plain state machine,
where the destination of each transition is solely determined by
the transition action and the origin state of the transition,
regardless of other preceding states before the origin.
For example, \texttt{KiF} \cite{kif} encodes a SIP system to a state machine,
% a context-free grammar ABNF \cite{abnf} to model SIP protocols,
\cite{snooze,mace} uses it to record network operation information,
and \cite{protocolstatefuzzing,tlsattacker} analysed state machine models of TLS implementations.
\texttt{PRISMA} \cite{prisma} defines the state machine model of the SUT in a probabilistic way
with a hidden Markov model \cite{hiddenmm},
which further labels each transition with its execution probability.
\texttt{PULSAR} \cite{pulsar} starts to improve \textsc{PRISMA}'s Markov model to the second order,
making the state/template selection depends on two preceding states.
\AFLNetLegion's tree model even more rigorously 
determines the next server state with all preceding states.
To mitigate potential state explosion problem,
\cite{testdatagen} with a rule-based state machine,
which prunes server states and transitions with pre-assumed rules,
e.g., ignoring state trajectories who are free from exceptions.
\AFLNetLegion's MCTS algorithm proposes a general and principled mitigation based on statistics 
without subjecting to such assumptions or domain knowledge.
Instead of pruning state space compartments from the model with rules, 
it prioritises expanding certain compartments based on execution statistics.
Its UCT algorithm estimates the structure of the server state space from past execution statistics
and guides its expansion in the state space accordingly.
Considering the uncertainty of the large state space,
its expansion not only prioritises the server states that appears to be promising to
further increase code coverage,
but also the states that are underexplored to
refine its estimation of their code structure.

In terms of learning these server models,
many techniques adopted manual learning,
which requires the specification of the state model \cite{boofuzz,sulley,peach,snooze}.
Although this improves the probability of generating valid queries,
the reliability of the model subjects to developers' understanding of the model and
the how well the specification describes the implementation.

To automate model learning,
passive learning is designed to train a model on a sufficient size data set
before fuzzing initiates.
Its efficiency and effectiveness rely heavily on the training set.
\textsc{PRISMA} \cite{prisma} proposed to cluster the network traffic sample to
infer a state machine of the SUT,
which also abstracts the query template from the sample traffic.
\textsc{PULSAR} \cite{pulsar} combines passive learning with fuzzing so that it can
generate queries from fuzzing templates with the state machine model and its embedded query rules.

Active learning is proposed as an alternative to passive learning,
for it does not rely on a large query corpus to initiate fuzzing.
For example, 
Angluin’s L* algorithm \cite{angluinl*} is an online algorithm to automate state inference
popular among several research works \cite{protocolstatefuzzing,mace,prospex}
to gradually infer a state machine model of the SUT through a number of queries.
As generative fuzzing techniques,
their query generation requires the SUT-specific query grammar and format.
In particular,
\cite{protocolstatefuzzing, mace} require a test harness to 
translate between abstract requests and actual packets;
While \cite{prospex} proposes to learn it automatically.
% \cite{testdatagen} screens mutation
% One concern of generative fuzzing is that many messages generated may not be valid.
An alternative to generate queries from templates is mutating known traces of real network traffic.
\AFLNet \cite{aflnet} takes advantage of this 
so that it can produce valid new queries at a high probability and
evolve from past interesting queries sequences.
Benefited from the same mutation-based strategy,
\AFLNetLegion can start fuzzing from any server state preferred.
To ensure the mutant are valid,
\cite{testdatagen} proposed to screen invalid queries
with a stateful rule tree that stores various query format requirements in layers.

Various kinds of server model learnt from different ways end up serving one goal:
Assisting selecting queries or query generation templates to generate new query sequences.
\textsc{PRISMA} \cite{prisma} corresponds each state to a template and 
randomly chooses one according to the transition probability of its Markov model.
\textsc{PULSAR} \cite{pulsar} has multiple templates in one state and 
prefers templates with more fuzz-able fields.
\textsc{MACE} \cite{mace} uses a priority queue to favour states traversed by past executions that 
visited a large number of unexplored basic blocks.
% \textsc{SNOOZE} \cite{snooze} leaves this burden to developers.
However, due to the complexity and uncertainty of external servers,
a query or a query template that appears boring may turn out to be rewarding in the long run. 
\AFLNet \cite{aflnet} uses an intuitive formula to consider candidates that are less often tested, 
trying to balance exploiting the benefit of candidates who appear interesting
with exploring the potential of the ones who seem to be boring.
\AFLNetLegion formalises this intuition with its MCTS algorithm.


% use active (snipuzz) / manual (snooze) learning for mutation 

% Focus of \AFLNetLegion:
% 1. Seed selection algorithm
% 2. Representation of the server (Tree vs. State Machine vs. Others)

% These papers seek to answer a different question under different settings.

% All of the papers use state machine to represent the server implementation.

% Most of them identify states in the same way that is different from \AFLNet and \AFLNetLegion.

% Many of them requires some preliminary information of the SUT, 
% e.g. a corpus of messages, test harness (grammar/abstraction of the messages), specification.

% Some of them focus on the implementation rather than algorithms.

% None of Them focuses on the seed selection algorithm.

% {\color{gray}
% \textbf{Peach}

% "Peach provides a way for one to define the format of data that should be generated and as well as how and when the fuzzed data should be generated."
% (From its documentation: https://wiki.mozilla.org/Security/Fuzzing/Peach)

% Peach cannot adjust seed selection and mutation strategies 
% according to runtime information of the program.
% (A Systematic Review of Network Protocol Fuzzing
% Techniques)
% }

% {\color{gray}
% \textbf{BooFuzz}

% No paper but a documentation of its functions and different types of message fields.
% Did not mention anything about algorithm or state representation.
% (From its documentation: https://buildmedia.readthedocs.org/media/pdf/boofuzz/latest/boofuzz.pdf)

% Use the specification of the protocol to construct
% the test inputs.
% (The Stacked Seq2seq-attention Model for Protocol Fuzzing)
% }

% {\color{gray}
% \textbf{SNOOZE}

% Focuses on the implementation of a tool rather than an algorithm.
% Described a lot about its primitives (data types, functions)
% "Alows a tester to describe the stateful operations of a protocol and 
% the messages that need to be generated."

% Represents SUT with a state machine.

% Requires to parse the specification of the provided protocol
% }


% \textbf{Protocol State Fuzzing of TLS Implementations}

% Blackbox fuzzing.

% Actively queries the the server implementation,
% and construct a state machine model based on the reponse.

% Learns the state machine with Angluin’s L* algorithm, 
% which is designed to learn a language (or Determinstic Finite Automata)
% via a number of queries.

% Requires a corpus of messages and a test harness to initiate.

% Focuses on state construction, instead of selection


% \textbf{Snipuzz}

% Blackbox fuzzing.

% Targets on Internet of Things (IoT), where the interaction is a bit different from external servers.

% Focuses on input mutation, rather than state modelling or input selection.

% For each message, 
% it attempts to mutate each byte of it (which creates a very large input space), 
% then clusters inputs based on the reponse,
% and merges clusers to reduce the input space.
% In this way, it learns which byte(s) are meaningful to mutate.

% Could be useful if we have zero knowledge of the grammar of syntax, 
% but not necessary in our case.


% {\color{gray}
% \textbf{TLS-Attacker}

% Focuses on the implementation of a tool rather than an algorithm.

% Aims to provide an easy-to-use framework with a simple user interface, 
% allowing developers to create custom TLS protocol ﬂows in order to discover state machine attacks.
% }


% \textbf{PULSAR}
% (published on SecureComm in 2015 (A in that year, C by now))

% Stateful Black-Box Fuzzing of Proprietary Network Protocols

% Infers a generative model for message formats and protocol states from network traffic.

% Uses \textbf{PRISMA}:
% They identify states in a different way from us.
% They start with a corpus of queries and responses,
% and categorise them into clusters.
% Then they infers the a Markov model of those clusters, and 
% build a query template with the model.


% \begin{figure*}[ht!]
%     \centering
%     % \input{case study - input seqs.tex}
%     \includegraphics[width=\linewidth]{Figures/prisma.png}
%     \vspace*{-.3cm}
%     \caption{PRISMA}
%     \label{fig: prisma}
% \end{figure*} 


% The method makes sense, but seems a bit counter-intuitive to me.
% Why would they tokenise query sequences and clusters them,
% instead of exactly record the sequence like \AFLNet did?

% The final output is similar: 
% Each state has a cluster of queries, 
% containing the server response code to the previous query and the next client query.

% \begin{figure*}[ht!]
%     \centering
%     % \input{case study - input seqs.tex}
%     \includegraphics[width=\linewidth]{Figures/pulsar.png}
%     \vspace*{-.3cm}
%     \caption{input clusters in each state}
%     \label{fig: pulsar}
% \end{figure*} 

% This paper represents the state machine of the protocol with a \emph{second order Markov model}.
% Unlike vanilla markov model 
% (where the destination of a transition purely depends on the origin),
% this model determines destination with two preceeding states.
% In that sense, it can be considered as a weaker version of our tree structure.


% {\color{gray}
% \textbf{Rule-Based State Machine}

% Uses state machine to describe the state of network protocol,
% uses a stateful rule tree to describe the relationship between states and messages.

% State machine: relies on the specification of a target network protocol.

% The  stateful rule tree: 
% different layers contains different kinds of information about the message,
% e.g. message types, message headers, specific requests.
% }

% {\color{gray}
% \textbf{KiF}
% Cited 75 times since published in 2005 on IPTComm

% Construct a state machine based on the grammar of SIP protocol,
% described with Augmented Backus–Naur form (ABNF) grammar.
% }



% \textbf{Conclusion}

% These papers might be useful if we want to expand the current work of \AFLNetLegion,
% e.g. try out different ways to identify each state, 
% or only to mutate certain parts of the queries or mutate with a collection of option



==> Sections/Threats.tex <==
\section{Threats to Validity}
\label{sec: aflnetlegion - threats}

\MYTODO{1. Implementations of AFLNet and AFLNetLegion, 2. generality of the 6 subjects.}
